Entropic optimal transport is maximum-likelihood deconvolution

We give a statistical interpretation of entropic optimal transport by showing that performing maximum-likelihood estimation for Gaussian deconvolution corresponds to calculating a projection with respect to the entropic optimal transport distance. This structural result gives theoretical support for the wide adoption of these tools in the machine learning community.

==> commands.tex <==

\usepackage{amsmath, amssymb, color}
\usepackage{amsthm} 
%\usepackage{natbib}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{xcolor,colortbl}
%
\RequirePackage{hypernat}
\usepackage{cleveref}
%
\usepackage{color}
\usepackage{amsfonts, fancybox}
\usepackage{amssymb}
\usepackage[american]{babel}
% \addto{\captionsamerican}{\renewcommand{\abstractname}{}}
%
\usepackage{psfrag,color}
\usepackage{dcolumn}
% \usepackage{subfigure}
\usepackage[format=hang, justification=justified, singlelinecheck=false]{subcaption}
\usepackage{flafter, bm, dsfont}
\usepackage[section]{placeins}
\usepackage[final]{showkeys}
\renewcommand*\showkeyslabelformat[1]{%
\fbox{\normalfont\tiny\ttfamily#1}}


\usepackage{multirow}
\usepackage{color}
\usepackage{amsmath}
\usepackage{float}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{amssymb}
%
%\usepackage{algorithmic, algorithm}
\usepackage{wrapfig}


\usepackage{amssymb, latexsym}

%
\usepackage{graphicx}
%
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{pgfplots}
\usepgfplotslibrary{fillbetween}

%% if you need to pass options to natbib, use, e.g.:
%% \PassOptionsToPackage{numbers, compress}{natbib}
%% before loading nips_2017
%%
%% to avoid loading the natbib package, add option nonatbib:
%%\usepackage[nonatbib]{nips_2017}
%
%%\usepackage[nonatbib]{nips_2017}
%
%% to compile a camera-ready version, replace the above line with the following, which has the [final] option, e.g.:
%% \usepackage[final]{nips_2017}
%
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{wrapfig}        % for wrapping figures
%\usepackage[notref, notcite, final]{showkeys}
%
%\usepackage{amsmath, amsthm, amsfonts}
%\usepackage{dsfont}
%\usepackage[sort]{cite}
%\usepackage{graphicx}
%
%% Notes
\usepackage{color}
\newcommand{\jw}[1]{{\textcolor{red}{[\textbf{JON:} #1]}}}
%\newcommand{\pr}[1]{{\textcolor{blue}{[\textbf{PR:} #1]}}}
%
%% For algorithms
\usepackage{algorithm}
%%\usepackage[noend]{algorithmic}
\usepackage[noend]{algcompatible}
%
%% Theorem definitions
\newtheorem{defin}{Definition}%[section]
\newtheorem{thm}{Theorem}%[section]
\newtheorem{exe}{Exercise}%[section]
\newtheorem{exa}{Example}%[section]
\newtheorem{fact}{Fact}%[section]
\newtheorem{prop}{Proposition}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{corol}{Corollary}%[thm]
\newtheorem{conj}{Conjecture}%[section]
\newtheorem{remark}{Remark}%[section]
\newtheorem{discussion}{Discussion}%[section]
\newtheorem{conc}{Conclusion}%[section]

% Custom definitions

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}


%\renewcommand{\subseteq}{\subset}

\newcommand{\R}{{\rm I}\kern-0.18em{\rm R}}
\newcommand{\h}{{\rm I}\kern-0.18em{\rm H}}
\newcommand{\PP}{{\rm I}\kern-0.18em{\rm P}}
\newcommand{\E}{{\rm I}\kern-0.18em{\rm E}}
\newcommand{\Z}{{\rm Z}\kern-0.18em{\rm Z}}
\newcommand{\1}{{\rm 1}\kern-0.24em{\rm I}}
\newcommand{\N}{{\rm I}\kern-0.18em{\rm N}}

\newcommand{\DS}{\displaystyle}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\Tr}{\mathrm{Tr}}

\newcommand*{\ep}{\varepsilon}
\newcommand*{\defeq}{:=}
\newcommand*{\dd}{\,\mathrm{d}}


\newcommand*{\Went}{W_{\sigma^2}}
\newcommand*{\Wentab}{\Went^{\alpha, \beta}}
\newcommand*{\Wentinf}{\Went^{1, \infty}}


